High-Performance Filters For GPUs

Filters approximately store a set of items while trading off accuracy for space-efficiency and can address the limited memory on accelerators, such as GPUs. However, there is a lack of high-performance and feature-rich GPU filters as most advancements in filter research has focused on CPUs. In this paper, we explore the design space of filters with a goal to develop massively parallel, high performance, and feature rich filters for GPUs. We evaluate various filter designs in terms of performance, usability, and supported features and identify two filter designs that offer the right trade off in terms of performance, features, and usability. We present two new GPU-based filters, the TCF and GQF, that can be employed in various high performance data analytics applications. The TCF is a set membership filter and supports faster inserts and queries, whereas the GQF supports counting which comes at an additional performance cost. Both the GQF and TCF provide point and bulk insertion API and are designed to exploit the massive parallelism in the GPU without sacrificing usability and necessary features. The TCF and GQF are up to $4.4\times$ and $1.4\times$ faster than the previous GPU filters in our benchmarks and at the same time overcome the fundamental constraints in performance and usability in current GPU filters.

==> characters.tex <==
%demo for special characters


\subsection{Type Changes and {\subsecit Special} Characters}
We have already seen several typeface changes in this sample.  You
can indicate italicized words or phrases in your text with
the command \texttt{{\char'134}textit}; emboldening with the
command \texttt{{\char'134}textbf}
and typewriter-style (for instance, for computer code) with
\texttt{{\char'134}texttt}.  But remember, you do not
have to indicate typestyle changes when such changes are
part of the \textit{structural} elements of your
article; for instance, the heading of this subsection will
be in a sans serif\footnote{A third footnote, here.
Let's make this a rather short one to
see how it looks.} typeface, but that is handled by the
document class file. Take care with the use
of\footnote{A fourth, and last, footnote.}
the curly braces in typeface changes; they mark
the beginning and end of
the text that is to be in the different typeface.

You can use whatever symbols, accented characters, or
non-English characters you need anywhere in your document;
you can find a complete list of what is
available in the \textit{\LaTeX\
User's Guide}\cite{Lamport:LaTeX}.



%and here is the stuff for theorems
\subsection{Theorem-like Constructs}
Other common constructs that may occur in your article are
the forms for logical constructs like theorems, axioms,
corollaries and proofs.  There are
two forms, one produced by the
command \texttt{{\char'134}newtheorem} and the
other by the command \texttt{{\char'134}newdef}; perhaps
the clearest and easiest way to distinguish them is
to compare the two in the output of this sample document:

This uses the \textbf{theorem} environment, created by
the \texttt{{\char'134}newtheorem} command:
\newtheorem{theorem}{Theorem}
\begin{theorem}
Let $f$ be continuous on $[a,b]$.  If $G$ is
an antiderivative for $f$ on $[a,b]$, then
\begin{displaymath}\int^b_af(t)dt = G(b) - G(a).\end{displaymath}
\end{theorem}

The other uses the \textbf{definition} environment, created
by the \texttt{{\char'134}newdef} command:
\newdef{definition}{Definition}
\begin{definition}
If $z$ is irrational, then by $e^z$ we mean the
unique number which has
logarithm $z$: \begin{displaymath}{\log e^z = z}\end{displaymath}
\end{definition}

Two lists of constructs that use one of these
forms is given in the

==> code/gqf_bulk_insert.tex <==
\begin{algorithm}[ht]
\caption{Bulk Inserts}
\label{alg:bulk-code}
\begin{algorithmic}[1]
\State $\textrm{slot\_per\_lock} \gets \textrm{gqf.slots\_per\_lock}$
\Function{Get\_Bucket\_Starts}{x[], buckets[]} \Comment{x is a sorted list of inputs, buckets is a an empty list of pointers}
\ForAll{buckets[i] in parallel}
    \State $minimum\_item \gets i \cdot slots\_per\_lock$ \Comment{find the minimum hash in the i-th locking region}
    \State \Call{Successor\_Search}{$minimum\_item$}
    \State \Return
\EndFor
\EndFunction
\State \Comment{The successor search looks for the smallest item greater than or equal to the queried item and returns the index of the item found}
\State

\State $\textrm{range} \gets \textrm{gqf.range}$ \Comment{GQF range variable} 
\Function{Hash\_All}{x[]}
\ForAll{x[i] in parallel}
    \State $x[i] \gets h(x[i]) \pmod{range}$
\EndFor
    \State \Return
\EndFunction
\State

\Function{Insert\_Even\_Odd}{buckets[], evenness}
    \ForAll{buckets[i] in parallel}
        \If{$i \pmod {2} = evenness$}
            \ForAll{item in buckets[i]}
                \State \Call{GQF\_INSERT}{$item$};
            \EndFor
        \EndIf
    \EndFor
    \State \Return
\EndFunction
\State

\State $\textrm{num\_locks} \gets \textrm{gqf.num\_locks}$
\Function{Bulk\_Insert}{x[]} \Comment{x is the list of input items}
    \State $buckets \gets malloc(num\_locks)$ \Comment{Allocate space for bucket }
    \State \Call{Hash\_All}{$x$}
    \State \Call{Sort}{$x$}  \Comment{Sorting is done using thrust::sort()}
    \State \Call{Get\_Bucket\_Starts}{$x, buckets$}
    \State \Call{Insert\_Even\_Odd}{$buckets, 0$}
    \State \Call{Insert\_Even\_Odd}{$buckets, 1$}
    \State \Return
\EndFunction

\end{algorithmic}
\end{algorithm}
\vspace{-1.0em}


==> figures.tex <==

\subsection{Figures}
This is a temporary placement for figures
These will eventually be moved to evaluation/other relevant sections.

\input{plots}

%temp placement of bulked comparisons between threads
\input{figures/aggregate_1_comparison}
\input{figures/aggregate_20_comparison}

\input{figures/20_20_comparison}
\input{figures/22_20_comparison}
\input{figures/24_20_comparison}
\input{figures/26_20_comparison}
\input{figures/28_20_comparison}





==> figures/gqf_variations.tex <==
\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{%
    \includegraphics{images/canonical_slots.png}
    }
    \caption{GQF structure visualized.}
    \label{fig:gqf_fig}
\end{figure}

==> quotient_filter.tex <==
\section{Counting quotient filter}\label{sec:qf-design}


In this section, we give an overview of Pandey et al.'s~\cite{PandeyBJP17a} counting \qf (CQF). We also describe the locking mechanism in the counting \qf for thread-safe operation because it acts as the building block in the \sysname (GQF). We finally explain how we design the counting quotient filter for the GPU.

%\item{Quotient Filters on the GPU have different bottlenecks than on the cpu}

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[height=0.6\columnwidth,width=0.8\columnwidth]{images/canonical_slots.png}
    \caption{The counting quotient filter~\cite{PandeyBJP17} structure. The upper part shows the canonical structure. The lower part shows the organization of the table in the quotient filter.}
    %It uses two metadata bits per slot. All items that share the same canonical location are stored together in a {\it run}. A sequence of items without any empty slot is called a {\it cluster}. Note: the items are showed in upper case in the canonical representation and the remainders corresponding to the items in the slots are showed in lower case.\steveinline{The fonts in this figure are tiny - need to increase them.}} 
    \label{fig:qf_structure}
    \vspace{-1.5em}
\end{figure}
\end{comment}

\subsection{CQF overview}

The counting quotient filter (CQF) stores an approximation of a multiset $S\subseteq \mathcal{U}$ by storing a compact, lossless representation of the multiset $h(S)$, where $h:\mathcal{U}\rightarrow\{0,\ldots,2^p-1\}$ is a hash function that maps items from the universe $\mathcal{U}$ to a $p$-bit fingerprint. To handle a multiset of up to $n$ distinct items while maintaining a false-positive rate of at most $\epsilon$, the CQF sets $p=\log_2 \frac{n}{\epsilon}$ (see the original quotient filter paper for the analysis~\cite{BenderFaJo12a}).

The \cqf uses Robin-Hood hashing~\cite{CelisLaMu85} to store the fingerprints compactly in a table. It consists of an array $Q$ of $2^q$ \defn{slots} and a hash function $h$ mapping items from a multiset to $p$-bit integers, where $p \geq q$.  Robin-Hood hashing is a variant of linear probing in which we try to place an item $a$ in slot $h(a) / 2^{p-q}$, but shift items down when there are collisions to create empty space. Robin-Hood hashing maintains the invariant that, if $h(a) < h(a')$, then $a$ will be stored in an earlier slot than $a'$.

The \cqf divides $h(x)$ into its first $q$ bits, \defn{quotient}
$h_0(x)$, and its remaining $r$ bits, \defn{remainder} $h_1(x)$.  It maintains an array $Q$ of $2^q$ $r$-bit slots, each of which can
hold a single remainder.  When an element $x$ is inserted, the \cqf
attempts to store the remainder $h_1(x)$ at index $h_0(x)$ in $Q$
(which we call $x$'s \defn{canonical slot}).  If that slot is already in
use, then the \cqf uses uses Robin hood hashing to find the next available empty slot to store $h_1(x)$. All the items that share the same canonical slot are stored together in a \defn{run} and a sequence of runs stored contiguously with no empty space is called a \defn{cluster}. During an insert operation, the next available empty slot is found at the end of the cluster. If an item lands at the start of the cluster then all the items in cluster must be shifted to create an empty space.

The \cqf also maintains 2 bits of additional metadata ({\it is\_occupieds} and {\it is\_runends}) per slot in order to determine which slots are in use and the canonical slot of each remainder stored in $Q$. When an item is inserted into the canonical slot, the {\it is\_occupieds} bit for that slot is set to 1. The {\it is\_runends} bit is set to one for every slot where the slot is occupied by an item that is the last remainder in a run. There is an one-to-one correspondence between {\it is\_occupieds} and {\it is\_runends} bit for every run. 
%Please refer to~\cref{fig:qf_structure}.

The queries maintain high lookup performance irrespective of the load factor\footnote{Load factor is the ratio of the number of occupied slots over the total number of slots in the filter}. Inserts still require shifts within the cluster, so insert performance does decrease as the load factor increases.

%The \cqf further maintains an extra 8 bits per block of 64 slots (called \defn{offset}) to speed up the operations to determine the start and end of each run during insertions and queries. Therefore, the total overhead due to metadata in a \cqf is 2.125 bits. In order to maintain good  performance, the array of slots cannot be filled beyond $95\%$. 
%We have omitted the offset bits in the \cqf block diagram in~\cref{fig:qf_structure} for simplicity.


%To quickly determine the start and end of a run the \cqf uses $RANK$ and $SELECT$ operations~\cite{PandeyBJP17a}. If the occupieds bit is set to 0 for a canonical slot then there is no item with that canonical slot in the table. If the occupieds bit is set to 1, then we can use the $RANK$ operation to determine the number of runs starting before this canonical slot and then perform the $SELECT$ operation to determine the end of the run, as there is a one-to-one correspondence between the occupieds and runends bit vector for each run.

%The \cqf supports efficient insertions, queries, updates, deletions, and hash enumeration just like any Robin-Hood hash table. It further supports efficient counting using a variable-length encoding of counters (see Pandey et al.'s paper~\cite{PandeyBJP17} for a detailed explanation). The counter encoding can also be used to associate small variable-size values with each hash in the table. Apart from the counter encoding, the \cqf also supports associating a small fixed-size value with each hash in the table. These values are stored along with the remainders in the table. To store the values, the table slots are resized to store the remainder and value together.

%The design of the GQF is based on the design of the Rank and Select Quotient Filter, or RSQF. The RSQF is a filter data structure that represents a set $S$ from a universe $U$ using a set of fingerprints. Let $f$ : $U \rightarrow [2^{p}]$ be a hash function that hashes elements of $U$ into $p$-bit fingerprints. Let $F = f(S) = \{f(x) | x \in S \}$ be te set of hash values of the elements of S. To perform an operation \textsc{LOOKUP(x)}, the filter checks whether $f(x) \in F$. The RSQF stores these fingerprints losslessy. Therefore, all false positive arise from collisions in the hash function, where $f(q) \in F$ for a query $q \not \in S$.

%To store an element from $F$, divide the $p$-bit hash value into its upper and lower bits. The quotient, $f_q(x)$, is comprised of the $q$ high-order bits, while the remainder $f_r(x)$ is comprised of the remaining $r = p - q$ low order bits. The fingerprint $f(x)$ is stored in the RSQF by inserting the remainder $f_r(x)$ into the $f_q(x)$th canonical slot. Although only $r$ bits per item are stored, the complete fingerprint can be recovered by recombining the remainder value and the slot number. 

%Remainders are stored in the RSQF in an array of length $2^q$. For each slot in the filter there are two metadata bits stored in a pair of bit arrays called the occupieds and runends. For an insert $f(q)$, the canoncial slot of the item is $f_q(x)$. All remainders are stored in sorted order, and if the canonical slot of an item is occupied, it may be shifted to the right. A group of elements with the same canonical slot $f_q(x) = f_q(y)$ will be stored in sorted order in contiguous slots and is called a run. A set of runs that occupy adjacent slots is called a cluster. 

%\subsection{Rank and Select operations}

%For a given slot $i$, $RANK(i)$ returns the number of 1s in a bit vector $B$ up to $i$, i.e. $RANK(B, i) = \sum_{x=0}^{i} B[x]$. $SELECT(i)$ performs the inverse operation, returning the index of the $i$th 1 in $B$. Together, $RANK$ and $SELECT$ allow us to quickly find the start and the end of the run associated with any item. If the occupieds bit is set to 0 for a canonical slot then there is no item with that canonical slot in the table. If the occupieds bit is set to 1, then we can use the $RANK$ operation to determine the number of runs starting before this canonical slot and then perform the $SELECT$ operation to determine the end of the run, as there is a one-to-one correspondence between the occupieds and runends bit vector for each run. 

%First, check if $occupieds[h_0(x)] == 0$ then there is no item with the given canonical slot. Otherwise, take the RANK(occupieds, $f_q(x)$). This will return the number of runs $b < f_q(x)$ in the filter up to slot $f_q(x)$. Given $t$ previous runs in the filter, we can use SELECT(runends, $t$) to find the slot corresponding to the end of the run associated with our canonical slot. 

%We scan backwards through this run until we either:

%\begin{enumerate}
%    \item Find a slot with remainder $h_1(x) == h_1(y)$
%    \item Reach a slot with a smaller remainder, ($h_1(x) < h_1(y)$
%    \item Reach the start of the run
%\end{enumerate}

%For queries, we return the true if $h_1(x) == h_1(y)$ for the found slot, and false otherwise. For inserts, the current slot is the correct slot for the insert, so we shift all items in the cluster one slot to the right, and insert into the current slot.

%To keep the $RANK$ and $SELECT$ operations local and cache efficient, the slots are organized into blocks of 64 slots, with an 8 bit offset value that tracks any overflows from previous blocks. 
%
%With the offsets, the work required to locate a run becomes highly efficient because we often only have to look in the current block and occasionally in the neighboring blocks if there is an overflow.

\subsection{Thread-safe counting quotient filter}

To perform thread-safe operations in the \cqf, explicit locks are maintained. To perform an insert operation, the thread needs to lock a big enough region so that shifting of items will not corrupt the subsequent region where another thread might be operating. Therefore, the slots are divided into locking regions that are big enough to handle the shifting of remainders during insertions without causing an overflow to the next locking region.

%In the \cqf, each locking region consists of 4096 slots. Each acquire a lock on the locking region where the canonical slot of the item it and the next region. Locking two consecutive regions in the \cqf ensure that even if during an insert operation we overflow into the next region it would still avoid memory corruption bugs.


%To safely write to a slot, we must lock both the run and all later runs in the cluster. In order to speed lock acquistion, the locks are affiliated with regions of the filter memory based on the maximum possible run size.

Given that the filter is only filled to 95\% load factor, we can safely say with that the maximum cluster size will be less than 8192 slots~\cite{GeilFO18}. In order to guarantee that each insert has at least this many slots to work with, we divide the filter into sections of 8192 slots. An insert thread grabs two locks corresponding to the canonical slot of the item and the lock immediately after it. Locking two consecutive regions in the \cqf ensures that memory corruption bugs are avoided, even if we overflow into the next region during an insert operation. The insert thread holds these locks until all changes are flushed to memory.
%
Similar locking mechanisms are used for the query and delete operations.

\begin{comment}

\subsection{Designing quotient filters for GPUs}

The main challenges in porting quotient filters to the GPU stem from the internal shifts required to insert new items into the filter. Large reads and writes to global memory are prohibitively expensive in CUDA and can dominate the run time at high load factors. As shown by Geil et al.~\cite{GeilFO18}, these shifts can be avoided if the entire dataset can be inserted in one batch. For many applications where filters are used, however, this is infeasible, as the dataset is either too large to fit within device memory or is passed to the device in batches. For these applications, the focus is instead to minimize the shifts caused by new data while guaranteeing that the filter remains internally consistent. Unlike a hash table, threads must retain ownership of an area larger than a single slot, as the shifts are too large to be performed with an atomic operation, and exclusive access to anything less than the entire shifted region can lead to corrupted metadata.
\end{comment}

==> refs.tex <==
\subsection{References}
Generated by bibtex from your ~.bib file.  Run latex,
then bibtex, then latex twice (to resolve references)
to create the ~.bbl file.  Insert that ~.bbl file into
the .tex source file and comment out
the command \texttt{{\char'134}thebibliography}.

==> table.tex <==
%a sample table

\begin{table*}
\centering
\caption{Some Typical Commands}
\begin{tabular}{|c|c|l|} \hline
Command&A Number&Comments\\ \hline
\texttt{{\char'134}alignauthor} & 100& Author alignment\\ \hline
\texttt{{\char'134}numberofauthors}& 200& Author enumeration\\ \hline
\texttt{{\char'134}table}& 300 & For tables\\ \hline
\texttt{{\char'134}table*}& 400& For wider tables\\ \hline\end{tabular}
\end{table*}

==> tables/api_table.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{c | c c | c c | c c | c c }
    \toprule
    Filter & 
    \multicolumn{2}{c}{{\bf Insert}} & \multicolumn{2}{c}{{\bf Query}} & \multicolumn{2}{c}{{\bf Delete}} & \multicolumn{2}{c}{{\bf Count}} \\
    \midrule
    & Point & Bulk  & Point & Bulk & Point & Bulk & Point & Bulk \\
    \midrule
    GQF & Yes & Yes  & Yes & Yes  & Yes & Yes  & Yes & Yes \\ 
    BF & Yes & Yes  & Yes & Yes  & No & No  & No & No \\ 
    SQF & No & Yes  & No & Yes  & No & Yes & No & No \\ 
    RSQF & No & Yes  & No & Yes  & No & No  & No & No \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{API supported by various filters. The GQF is the only filter that supports a range of operations. RSQF can support deletes but it is not implemented by the authors.}
    \label{tab:api_table}
    \vspace{-1.5em}
\end{table}


==> tables/bulk_insert.tex <==
\begin{algorithm}[ht]
\caption{Bulk Inserts}
\label{alg:bulk_inserts}
\begin{algorithmic}
\State $\textrm{slot\_per\_lock} \gets \textrm{gqf.slots\_per\_lock}$
\Function{Get\_Bucket\_Starts}{x[], buckets[]} \Comment{x is a sorted list of inputs, buckets is a an empty list of pointers}
\ForAll{buckets[i] in parallel}
    \State $minimum\_item \gets i \cdot slots\_per\_lock$ \Comment{find the minimum hash in the i-th locking region}
    \State \Call{Successor\_Search}{$minimum\_item$}
    \State \Return
\EndFor
\EndFunction
\State \Comment{The successor search looks for the smallest item greater than or equal to the queried item and returns the index of the item found}
\State

\State $\textrm{range} \gets \textrm{gqf.range}$ \Comment{GQF range variable} 
\Function{Hash\_All}{x[]}
\ForAll{x[i] in parallel}
    \State $x[i] \gets h(x[i]) \pmod{range}$
\EndFor
    \State \Return
\EndFunction
\State

\Function{Insert\_Even\_Odd}{buckets[], evenness}
    \ForAll{buckets[i] in parallel}
        \If{$i \pmod {2} = evenness$}
            \ForAll{item in buckets[i]}
                \State \Call{GQF\_INSERT}{$item$};
            \EndFor
        \EndIf
    \EndFor
    \State \Return
\EndFunction
\State

\State $\textrm{num\_locks} \gets \textrm{gqf.num\_locks}$
\Function{Bulk\_Insert}{x[]} \Comment{x is the list of input items}
    \State $buckets \gets malloc(num\_locks)$ \Comment{Allocate space for bucket }
    \State \Call{Hash\_All}{$x$}
    \State \Call{Sort}{$x$}  \Comment{Sorting is done using thrust::sort()}
    \State \Call{Get\_Bucket\_Starts}{$x, buckets$}
    \State \Call{Insert\_Even\_Odd}{$buckets, 0$}
    \State \Call{Insert\_Even\_Odd}{$buckets, 1$}
    \State \Return
\EndFunction


==> tables/percentiles.tex <==
\begin{table}[t]
\centering
    \begin{tabular}{| c | c | c | c | c | c |}
    \toprule
    {\bf Percentile} & 50 & 99 & 99.9 & 99.99 & Max \\
    \midrule 
    {\bf Cluster Size} & 4 & 492 & 1402 & 2594 & 8114 \\
    \bottomrule
    \end{tabular}
    \caption{Distribution of cluster size in a GQF with $2^{28}$ slots filled at 95\% load factor. The data was collected over 20 runs.}
    \label{tab:cluster-percentile}
    \vspace{-1.5em}
\end{table}


==> tables/performance_breakdown.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{| c | c | c | c | c |}
    \toprule
    {\bf Insertion phase} & Hash & Sort & Get Bucket Starts & Insert Buffers \\
    \midrule 
    {\bf Percentage of Run Time} & 2.231\% & 13.705\% & .027\% & 84.038\% \\
    \bottomrule
    \end{tabular}
    }
    \caption{Percentage breakdown of different phases during bulk insertion in the GQF with $2^{28}$ slots.}
    \label{tab:insertion-breakdown}
    \vspace{-1.5em}
\end{table}
